Multi-level Consistency Learning for Semi-supervised Domain Adaptation

Semi-supervised domain adaptation (SSDA) aims to apply knowledge learned from a fully labeled source domain to a scarcely labeled target domain. In this paper, we propose a Multi-level Consistency Learning (MCL) framework for SSDA. Specifically, our MCL regularizes the consistency of different views of target domain samples at three levels: (i) at inter-domain level, we robustly and accurately align the source and target domains using a prototype-based optimal transport method that utilizes the pros and cons of different views of target samples; (ii) at intra-domain level, we facilitate the learning of both discriminative and compact target feature representations by proposing a novel class-wise contrastive clustering loss; (iii) at sample level, we follow standard practice and improve the prediction accuracy by conducting a consistency-based self-training. Empirically, we verified the effectiveness of our MCL framework on three popular SSDA benchmarks, i.e., VisDA2017, DomainNet, and Office-Home datasets, and the experimental results demonstrate that our MCL framework achieves the state-of-the-art performance.

==> table/augmentation.tex <==
\begin{table}[!htbp]
    \centering
    % \vspace{-2mm}
    \scalebox{0.92}{
        \begin{tabular}{cccc}
        \toprule
        $x^{A}$
        & $x^{B}$
        & R $\rightarrow$ C
        & R $\rightarrow$ S \\
        \midrule
        Strong &  Strong & 74.9 & 65.1\\
        Strong &  Weak & 61.0 & 55.2 \\
    Weak &  Weak & 72.3 & 63.9 \\
Weak &  Strong & \textbf{77.4} & \textbf{70.7} \\
        \bottomrule
        \end{tabular}
    }
    \vspace{2mm}
    \caption{Accuracy w.r.t. augmentation strategies in task R $\rightarrow$ C and R $\rightarrow$ S on \textit{Domainnet}.}
    \label{table:augmentation}
\end{table}

==> table/multiple.tex <==
\begin{table}[!htbp]
    \centering
    % \vspace{-2mm}
    \scalebox{1.0}{
        \begin{tabular}{lcccccccc}
        \toprule
        \small \textbf{Method}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ C}
        &  \small \rotatebox[origin=c]{0}{P $\rightarrow$ C}
        &  \small \rotatebox[origin=c]{0}{C $\rightarrow$ S}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ P}
        &  \small \rotatebox[origin=c]{0}{S $\rightarrow$ P}
        &  \small \rotatebox[origin=c]{0}{R $\rightarrow$ S}
        & \small \textbf{Avg} \\  
        \midrule
        STD & 0.3 & 0.4 & 0.2 & 0.6 & 0.7 & 0.2 & 0.4 \\
        \bottomrule
        \end{tabular}
    }
    \caption{Standard deviation of Accuracy over five runs on \textit{Domainnet} in the 3-shot setting. Note that \textbf{Avg} denotes the standard deviation of the mean accuracy over five runs.}
    \label{table:multiple_run}
\end{table}

==> table/res_ablation.tex <==
\begin{table}[t]
    \centering
    \caption{ Ablation studies (\%) on \textit{VisDA2017} under the settings of 1-shot and 3-shot using a ResNet34 backbone. }
    \label{res_ablation}
    % \vspace{-2mm}
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{
        >{\centering\arraybackslash}p{0.6cm}|
        >{\centering\arraybackslash}p{1cm}
        >{\centering\arraybackslash}p{1cm}
        >{\centering\arraybackslash}p{1cm}
        >{\centering\arraybackslash}p{1cm}|
        >{\centering\arraybackslash}p{1cm}
        }
        \toprule
        & $\mathcal{L}_{CE}$
        & $\mathcal{L}_{PL}$
        & $\mathcal{L}_{cross}$
        & $\mathcal{L}_{intra}$
        & \textbf{MCA} \\ 
        \midrule
        \multicolumn{6}{c}{\textbf{One-shot}}\\
        \midrule
        ($a$) & \checkmark  &  & \checkmark  &  &  78.9  \\
        ($b$) & \checkmark  &   &  & \checkmark &  77.0  \\
        ($c$) & \checkmark  &   & \checkmark & \checkmark &  79.7  \\
        ($d$) & \checkmark  & \checkmark & \checkmark &  &  83.5  \\
        ($e$) & \checkmark  & \checkmark &  & \checkmark &  82.4  \\
        ($f$) & \checkmark  & \checkmark  & \checkmark  & \checkmark  &  86.3  \\
        \midrule[0.7pt]
        \multicolumn{6}{c}{\textbf{Three-shot}}\\
        \midrule
        ($g$) & \checkmark  &  & \checkmark  &  &  79.8  \\
        ($h$) & \checkmark  &   &  & \checkmark &  78.3  \\
        ($i$) & \checkmark  &   & \checkmark & \checkmark &  80.5  \\
        ($j$) & \checkmark  & \checkmark & \checkmark &  &  83.8  \\
        ($k$) & \checkmark  & \checkmark &  & \checkmark &  84.6  \\
        ($l$) & \checkmark  & \checkmark  & \checkmark  & \checkmark  &  87.3  \\
        \bottomrule
        \end{tabular}
    }
    % \vspace{-3mm}
\end{table}

==> table/res_hyper2.tex <==
\begin{table}[t]
    \centering
    \caption{Accuracy w.r.t. loss weight $\lambda_2$ on C $\rightarrow$ P of \textit{Office-Home} 3-shot setting given $\lambda_1 = 1$.}
    \vspace{-2mm}
    \resizebox{0.82\linewidth}{!}{
        \begin{tabular}{
        >{\centering\arraybackslash}p{1.5cm}|
        >{\centering\arraybackslash}p{1.cm}
        >{\centering\arraybackslash}p{1.cm}
        >{\centering\arraybackslash}p{1.cm}
        >{\centering\arraybackslash}p{1.cm}
        }
        \toprule
        $\lambda_1$ & 0 & 0.1 &  0.2 &  0.5 \\
        \midrule
        Accuracy & 82.0 & 83.5 & 84.3 & 84.0\\
        \bottomrule
        \end{tabular}
    }
    \label{table:loss_weight_2}
\end{table}

==> table/res_hyper3in1.tex <==
\begin{table}[t]
    \centering
    % \vspace{-2mm}
    \scalebox{0.82}{
        \begin{tabular}{lcccc}
        \toprule[1.2pt]
        $\lambda_1$ & 0 & 0.5 &  1.0 &  1.5 \\
        \midrule[0.3pt]
        Accuracy & 82.9 & 83.5 & 84.3 & 83.6 \\
        \midrule[0.7pt]
        $\lambda_2$ & 0 & 0.1 &  0.2 &  0.5 \\
        \midrule[0.3pt]
        Accuracy & 82.0 & 83.5 & 84.3 & 84.0\\
        \midrule[0.7pt]
        $T$ & 0.75 & 1.0 &  1.25 & 1.5 \\
        \midrule[0.3pt]
        Accuracy & 81.7 & 83.9 & 84.3 & 82.3 \\
        \bottomrule[1.2pt]
        \end{tabular}
    }
     \caption{Accuracy w.r.t. 3 hyper-parameters, loss weight $\lambda_1, \lambda_2$ and the softmax temperature $T$, on C $\rightarrow$ P of \textit{Office-Home} 3-shot setting. Note the default setting is $\lambda_1 = 1$, $\lambda_2 = 0.2$, and $T = 1.25$, and in each group of ablative experiments we only change one hyperparameter in the default setting. }
    \label{table:hyper3in1}
\end{table}

==> table/res_hyperparam.tex <==
\begin{table}[t]
    \centering
    \caption{Accuracy w.r.t. loss weight $\lambda_1$ on C $\rightarrow$ P of \textit{Office-Home} 3-shot setting given $\lambda_2 = 0.2$.}
    \vspace{-2mm}
    \resizebox{0.82\linewidth}{!}{
        \begin{tabular}{
        >{\centering\arraybackslash}p{1.5cm}|
        >{\centering\arraybackslash}p{1.cm}
        >{\centering\arraybackslash}p{1.cm}
        >{\centering\arraybackslash}p{1.cm}
        >{\centering\arraybackslash}p{1.cm}
        }
        \toprule
        $\lambda_1$ & 0 & 0.5 &  1 &  1.5 \\
        \midrule
        Accuracy & 82.9 & 83.5 & 84.3 & 83.6 \\
        \bottomrule
        \end{tabular}
    }
    \label{table:loss_weight_1}
\end{table}

==> table/res_uda.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.65}{
        \begin{tabular}{l|c}
        \toprule
        \textbf{Method} & \textbf{MCA} \\
        \midrule
        S+T & 49.2 \\
        MME  & 63.4 \\
        MCC & 69.8 \\
        CDAN $+$ MCC & 72.5 \\
        \midrule 
        \textbf{MCL} & \textbf{82.7}   \\
        \bottomrule
        \end{tabular}
    }
    \caption{Mean Class-wise Accuracy(\%) on \textit{VisDA2017} UDA setting using ResNet34 as the backbone.}
    \label{res_uda}
    \vspace{2mm}
\end{table}

==> table/temp.tex <==
\begin{table}[t]
    \centering
    \caption{Accuracy w.r.t. softmax temperature $T$ for thresholding on \textit{Office-Home} 3-shot setting.}
    \vspace{-2mm}
    \scalebox{0.82}{
        \begin{tabular}{lcccc}
        \toprule
        $T$ & 0.75 & 1 &  1.25 & 1.5 \\
        \midrule
        Accuracy &  &  &  & \\
        \bottomrule
        \end{tabular}
    }
    \label{table:temp}
\end{table}
